Pre-Trained Multilingual Sequence-to-Sequence Models: A Hope for Low-Resource Language Translation?

What can pre-trained multilingual sequence-to-sequence models like mBART contribute to translating low-resource languages? We conduct a thorough empirical experiment in 10 languages to ascertain this, considering five factors: (1) the amount of fine-tuning data, (2) the noise in the fine-tuning data, (3) the amount of pre-training data in the model, (4) the impact of domain mismatch, and (5) language typology. In addition to yielding several heuristics, the experiments form a framework for evaluating the data sensitivities of machine translation systems. While mBART is robust to domain differences, its translations for unseen and typologically distant languages remain below 3.0 BLEU. In answer to our title's question, mBART is not a low-resource panacea; we therefore encourage shifting the emphasis from new models to new data.

==> not used/1.introduction.tex <==
\section{Introduction}
%\eal{My suggestion is that we don't give a tutorial about the existing methods, it is expected the ACL audience would already have this knowledge.  So you might want to move this short history lesson to Appendix.  So we can move the first two paragraphs, very well written history.}
%Transformer based self-supervised embedding models have changed the trajectory of the field of Natural Language Processing (NLP) into a new dimension. Their power lies in self-supervised pre-training, meaning that these models are trained with un-annotated data only. 
%Currently available self-supervised embedding models can be broadly categorised into three pats: (1) Those that train an encoder transformer model using an objective such as masked token prediction or next sentence prediction (e.g.~BERT [], RoBERTA []), (2) Those that train a decoder transformer model for next word prediction (e.g. GPTx []), and (3) Those that train an encoder-decoder transformer  model using a denoising objective (e.g.~BART [], T5[]). While the type of NLP tasks implemented by these models cannot be distinctly categorised, each type of model has been a preferred choice for sub-set of NLP tasks. The first type of models are commonly used for tasks such as text classification and information extraction. The second type of models are used for tasks such as text generation and question answering. The third type of models are used for tasks such as Machine Translation and text summarization.
The sudden need to translate basic health tips into various languages during global medical emergencies, such as the COVID-19 pandemic ~\cite{DBLP:journals/corr/abs-2104-05848}, is a crucial area of inequity for marginalized communities.  Data-hungry neural machine translation models perform poorly on low-resource languages (LRL) \eal{citation needed} because they are typically trained on high-resource languages (such as English, French, German) and on open domain corpus like news, books, blogs and Wikipedia.  Adapting these machine translation models do not generalize well to specific domains such as public health, which contain scientific terms that may be absent in indigeneous languages.  Therefore, \eal{...mention our contribution here}.

% \eal{move to appendix, very much detract from the storyline; no domain-specific health trianing data used}
% All these are realistic scenarios. Borrowing the example given by~\cite{zhou2021family}, there can be a scenario where Covid-19 related health guidelines available in English to be translated to multiple low-resource languages. This translation task is domain-specific, and the available parallel data for the considered languages may just be domain-specific data such as the Bible data. Or the considered low resource language may not have any parallel data at all, and parallel data has to be extracted from open-domain web sources using some parallel corpus mining technique. 


%\eal{Need to add background introducing the problem/task at hand, which is MT:  Instead of a history lesson, can we try starting with MT for LRL and why this is an important problem?  The COVID19 example is appropriate here to open the paper; but maybe to make the paper more relevant through time and lasting through the ages, we could just say something more generic like "pandemic medical advice in different languages"}

%\rs{can we shrink the above to a shorter version like this? We probably want to open the introduction quickly and specifically on mBART. Because we want to introduce our evaluation factors to uncover the reason behind mBART at front, too. } 
%Recent works have been focusing on large-scale multilingual language models to improve performance on several NLP tasks\rs{cite}. In multilingual machine translation, low-resource languages can benefit from models jointly trained in the multilingual setting with shared representations \rs{Gu et al.,
%2018)}. mBART50~\cite{liu-etal-2020-multilingual-denoising}, a multilingual sequence-to-sequence denoising auto-encoder trained on large unlabeled monolingual corpora across 50 languages \rs{cite}. 

%\eal{Literature Review and SoTA flaws: Can this part be specific the multiNMT, especially empirical studies involving mBART50 and/or MT5? } Subsequently, different studies have been carried out to identify the capabilities of these models under different settings such as different pre-training data set sizes [], different fine-tuning dataset sizes [] and different levels of language similarity []. However, such extensive experiments have been carried out only for the first type of models mentioned above, namely mBERT and XLM-R. Evaluations of sequence-to-sequence models such as mBART and mT5 have been limited to the research that introduced these models [need to verify this]. Despite this dearth, these models have shown very promising results for low resource languages for tasks such as Machine Translation [], and text summarization [].\eal{can we focus on MT and not mention summarization?}

%\eal{a sentence here about what missing in existing literature and how we solve that:  There has been no previous large-scale empirical study on mBART50 especially studying the factors that effect LRL NMT.}

%\subsection{Problem Definition}
%\citet{muller-etal-2021-unseen}
%\citet{ebrahimi-kann-2021-adapt}

\eal{the meat of our work starts here, emphasize this!}
We present the first large-scale study of MT using multilingual pre-trained sequence-to-sequence models. We consider the problem of data scarcity faced by low-resource languages and analyse the performance of pre-trained NMT models when fine-tuned with the  use of publicly available parallel data. We selected mBART50 model, as it is the most used model for Machine Translation, plus it has been reported to perform better on average, when compared to mT5~\cite{liu2021continual}. \\
Our analysis is guided by the observation that the publicly available parallel datasets for Machine Translation (MT)~\cite{tiedemann-thottingal-2020-opus} can be broadly categorised as (1) high quality datasets, which are small in size and are mostly domain-specific, and (2) Automatically extracted from public domain documents in the web, which are large in size but very much noisy. In this study, we investigate the capability of these pre-trained models to produce robust 
% \eal{multi-}\st{shouldn't be multi-NMT, each direction is trained as separate bilingual manner}\eal{ok, resolve}
NMT  models for low resource languages, when fine-tuned with small amounts of manually curated domain-specific data as well as comparatively large amounts noisy parallel data. Both types of fine-tuning have been tested with domain-specific, as well as open domain test data. Given that mBART50 covers only 50 languages, we investigate the possibility of using mBART for languages not included in pre-training. 
% \eal{maybe too much detail?  perhaps we can generally explain the contribution of our work in the intro and go into the logical details of the choices in the methodology}


We carry out an in-depth evaluation of the cross-lingual transfer abilities of the mBART50 model in the context of low-resource languages. We consider the impact of the following factors on mBART50 performance: 
\begin{enumerate}
    % \item mBart of LRL
    \item Data Efficiency:  Size of the fine-tuning dataset for the low-resource language;  
    \item mBart Pre-Training:  Amount of data used in pre-training the mBART50 model; 
    % \item Typological relationship between languages; and 
    \item Noisiness of parallel data used for fine-tuning, whether it is automatically curated or carefully hand-crafted.
    \item Corpus Relatedness:  Domain-relatedness of the test dataset and the fine-tuning dataset; 
\end{enumerate}

% Our empirical analysis \eal{?results?} shows that .........

The contributions of this paper is in 3-folds:  1) extreme LRL originating from South Asia (si, a, ka, as) and Africa (af, xh, yo, 2) empirical evidence on factors effecting mBart fine-tuning (transfer learning) of LRL (domain-specific fine-tuning, amount of data needed, generic open-domain fine-tuning, in/not-in mbart) 3)recommendations on leveraging these factors for mBart of LRL


==> not used/2.method.tex <==
% \section{Problem Definition}
% \label{method}
% This section discusses the problem of fine-tuning pre-trained NMT models on low-resource languages with scarce data. 
% \citet{muller-etal-2021-unseen}

% \citet{ebrahimi-kann-2021-adapt}

% \subsection{Related Work}\eal{need to also merge with Surangika's Related Work at the end; we will decide whether this come in the beginning or the end...given the lengthiness of the 4 subsections, probably the end is appropriate so that we don't distract the reader from our work}


\subsection{Domain Relatedness}
% \rs{For consistency with the discussion, should we also put explanation of domain relatedness and why we should keep track of this when analyzing our exp results?}\eal{thank you, I will do this}
%language relatedness plays a major role in pre-trained multilingual models such as mBERT [], as well as multilingual NMT models []. \sr{how we quantified this should come here}


Recent literature in domain adaptation focusing on language models found that there domains can be clustered and separated \cite{aharoni2020unsupervised}; however, these works do not explore extreme low-resource languages, especially low-resource South Asian and African languages \cite{ustun2021multilingual, ko2021adapting}.  


\subsection{Language Relatedness}
Previous works suggest that zero-shot cross-lingual transfer on low resource languages is improved when the multilingual language model has seen a related language during pretraining~\cite{zhou-etal-2018-massively, DBLP:journals/corr/abs-2004-13939, muller-etal-2021-unseen,  DBLP:journals/corr/abs-2104-05848}. 

TODO: explain WALS, genetic vs. syntactic, and we will use this to analyze the fine-tuned mBART performance to conclude that the data factors drive the force of this, which subsequently impact the performance in cross-lingual transfer.



==> not used/2.sequence-to-sequence-models.tex <==
\section{Literature Review / Related Work - Sequence-to-Sequence Pre-trained Models}
\eal{surangika - my preference is to either make this very short (1 paragarph) or move it to before the conclusion; I think this depends on the strength of the literature in supporting our contributions (what is missing in current work and how we fill that need)}

Transformer based self-supervised embedding models have changed the trajectory of the field of Natural Language Processing (NLP) into a new dimension. Particularly, multilingual pre-trained embedding models such as mBERT~\cite{devlin2019bert}, XLM-R~\cite{conneau2019unsupervised}, as well as mBART~\cite{liu2020multilingual} and mT5~\cite{xue-etal-2021-mt5} have shown very promising results in the context of low resource languages.

While encoder-based multilingual models such as mBERT and XLM-R have been subjected to extensive empirical evaluations~\cite{muller2021being, wu2020all, wu2019beto}, the same (surprisingly) does not hold for multilingual sequence-to-sequence denoising autoencoder models such as mBART or mT5. Despite this dearth, these autoencoder models have delivered impressive results for NLP tasks such as Machine Translation (MT), Text Generation, and Text Simplification~\cite{fan2021beyond, gonzales2021new}. Their performance on Machine Translation of low resource languages~\cite{thillainathan2021fine} is of particular interest, as Machine Translation for low-resource languages has been long identified as a very challenging problem~\cite{ranathunga2021neural}. However, the past work that utilized these multilingual sequence-to-sequence models for MT~\cite{ustun2021multilingual, fan2021beyond, liu2021continual} has not provided a comprehensive analysis on how the result of their fine-tuning is constrained on competing factors such as pre-training dataset size, fine-tuning dataset size, domain-relatedness or language relatedness.



%The initial self-supervised models were trained on a monolingual setting. However, building self-supervised embedding models for each distinct language is a costly operation, plus certain low resource languages may not have enough data to train these models. As a natural solution, multilingual self-supervised pre-trained models emerged. While BERT and RoBERTA have their multilingual models as mBERT [] and XLM-R[], respectively, BART and T5 have mBART [] and mT5 [] (respectively). These multilingual models have demonstrated impressive results particularly for zero-shot and few-shot scenarios.


\sr{sarubi- shall we try to improve this section a bit? looking at related papers on mBART would help. also it is nice to have some citations}\eal{see the above 2 paragraph moved from introduction}
The state-of-the-art sequence-to-sequence pre-trained models are trained in a self-supervised manner using large-scale monolingual data; here, the monolingual data is noised and fed as a source task and original monolingual data as the target task. At the end of the self-supervised training, the trained model can take a partially noised input and predict the denoised words to recover the original sentence.  This approach strongly learns a good universal language representation from the monolingual data by capturing linguistic characteristics, lexical meanings, and syntactic and semantic structures. 

\sr{i think we should first introduce BART and then mBART}
The first trained complete sequence-to-sequence model is BART \cite{lewis2019bart}. It is implemented as a standard sequence-to-sequence Transformer architecture with a bidirectional auto-encoder and a left-to-right auto aggressive decoder. Hence, it comprises two pre-trained models, a bidirectional encoder similar to BERT~\cite{devlin2019bert}, and a left-to-right decoder similar to GPT~\cite{radford2018improving_gpt}. It is purely trained on large scale English monolingual data. Later this BART has expanded with multiple monolingual data and trained similarly as a single model. 

mBART~\cite{liu2020multilingual_mbart25} is a prominent multilingual sequence-to-sequence pre-trained model, and the first of its kind. It is simply the multilingual version of the BART (Bidirectional and Auto-Regressive
Transformers) model~\cite{lewis2020bart}. The mBART \cite{tang2020multilingual_mbart50} model has been pre-trained with 50 languages. For noising the input texts, mBART has applied techniques such as random span masking and order permutation.  
\sr{David - a little bit on mT5}



==> not used/5.discussion.tex <==
\section{Discussion}


\newpage\newpage
\section{Appendix}
\subsection{Discussion on Language Relatedness}
\sr{Roslin - i think this discussion should be moved to section . then we can refer it here, and discuss whether results shown any dependence on language/domain relateness}
\begin{itemize}
    \item Language relatedness did not seem to be driving the performance with the unseen cases:
    \item Yoruba: syntax is similar to Xhosa (~0.65), and phonology similar to Tamil, Telugu, and Xhosa (above 0.7)
    \item Kannada: syntax is similar to Telugu, Tamil, Sinhala, Assamese (above 0.8), phonology is similar to Sinhala, Assamese, Bengali, and Tamil (0.94)
    \item Yoruba was actually better in terms of performance? Maybe it is less similar to the other ones, that the model will actually shift it's weights towards the new language? Do we have quanlitative analysis of Yoruba/Kannada outputs? Do they borrow scripts from other langs?
    \item \eal{Rosaline:  can we explain why french performs worse? and afrikan have such good results}
\end{itemize}

\subsection{Discussion on Domain Relatedness}

In order to get an understanding of the relatedness of different domains, we....
\eal{TODO:  add more comments with Shravan and David}
Domain type indicates whether the dataset is domain-generic or domain-specific. This factor is crucial to differentiate the model's performance on the domain adaptation task. To evidently show the strength of domain type, we select four datasets from specific domains: Bible, government communications, legislation, and \sr{shraven - what is the domain of Indic datasets}.\sr{Annie- domain relatedness discussion should come here}\eal{I put domain relatedness discussion in discussion after results for now \href{https://docs.google.com/document/d/103eYp5iXchKwNuOP9m0d_zh7iXYOQusq_2YV-N3gyv8/edit#heading=h.ecr6mvph3qxa}{Domain Relatedness Literature Review link};  \href{https://docs.google.com/presentation/d/10wukbff-Ko5wwo6wAIVZBUiZXCKy0unSrMA3ULdR0Co/edit#slide=id.gfce37dd943_0_0}{Domain Relatedness discussion link}} \rs{can we actually introduce domain relatedness in Section \ref{method}, and refer to that section in here?} \href{https://docs.google.com/document/d/103eYp5iXchKwNuOP9m0d_zh7iXYOQusq_2YV-N3gyv8/edit#heading=h.ecr6mvph3qxa}{Literature Review};  \href{https://docs.google.com/presentation/d/10wukbff-Ko5wwo6wAIVZBUiZXCKy0unSrMA3ULdR0Co/edit#slide=id.gfce37dd943_0_0}{Analysis}\eal{conclusion: wait for experimental results and analyze to see if there is correlation, if no impact don't introduce}


\begin{figure}[h]
\includegraphics[width=8cm]{images/domain_relatedness_allcombined.png}
\end{figure}

\begin{figure}[h]
\includegraphics[width=8cm]{images/domain_relatedness_ccalign.png}
\end{figure}

\begin{figure*}[h]
\includegraphics[width=16cm]{images/domain_relatedness_heatmap.png}
\end{figure*}

\begin{figure*}[h]
\includegraphics[width=14cm]{images/domain_relatedness_allseparate.png}
\end{figure*}

==> not used/6.literature.tex <==
\section{Related Work}
\subsection{Evaluating Pre-Trained Multilingual Models}
\subsubsection{Encoder-based Multilingual Models}
The language and task agnostic capabilities of pre-trained multilingual models make their evaluation a tedious task. An ideal in-depth evaluation would have to consider multiple competing pre-trained models, across multiple languages, multiple tasks, multiple fine-tuning dataset sizes, etc. Further analysis has to be carried out with respect to factors such as language relatedness, the amount of data used in the pre-trained models,  and the domain and type of the data used for fine-tuning. 

While we are not aware of any in-depth empirical analysis of sequence-to-sequence pre-trained models  considering these different factors, much research can be found for encoder based multilingual models such as mBERT and XLM-R. However,  the past work on evaluating these models have been focusing only on a sub-set of the aforementioned different competing aspects. 

When introducing a new multilingual dataset for a particular task, it is a common practice to present benchmark results using multiple pre-trained models~\cite{li-etal-2021-mtop}. On the other hand, when introducing a novel multilingual pre-trained model, this model is compared against the existing models over multiple languages and tasks~\cite{artetxe2020cross}. There have also been many empirical studies that examined the zero-shot and few-shot capabilities of these models~\cite{hu2020xtreme, lauscher2020zero},  as well as how they perform under specialized settings such as code-mixed data~\cite{aguilar-etal-2020-lince} or unseen languages~\cite{ebrahimi-kann-2021-adapt}. There have been experiments to understand how factors such as pre-trained dataset size~\cite{acs2021evaluating}, language relatedness~\cite{lauscher-etal-2020-zero}, level of the NLP task~\cite{lauscher-etal-2020-zero}, and model properties~\cite{raganato-etal-2020-xl} affect the end result. It has been a common observation that typological relatedness of languages plays a noticeable role when low-resource are involved~\cite{lauscher2020zero,wu2020all}.~\citet{wu2020all} showed that for languages under-represented in the pre-trained models, fine-tuning with small amounts of labelled data (few-shot)  is not effective. On the other hand,~\citet{hu2020xtreme}  showed that for low resource languages, zero-shot can deliver better results than few-shot, when the latter is fine-tuned with a large amount of English data. This contradicts with~\citet{lauscher-etal-2020-zero}, who showed substantial improvements of few-shot over zero-shot.~\citet{ebrahimi2021americasnli} showed that zero-shot is harder for unseen languages, while~\citet{ebrahimi-kann-2021-adapt} showed that this can be alleviated by techniques such as continuous pre-training. 

\subsubsection{Sequence-to-sequence Multilingual Models}
Research that introduced different sequence-to-sequence pre-trained models and different fine-tuning techniques have carried out limited analysis on how these models behave under different circumstances.~\cite{liu2020multilingual} showed that the mBART25 model fails to deliver meaningful results when fine-tuning with less than 10k sentences. The performance has also dropped when fine-tuned with 25M sentences. They showed that pre-training on more languages helps most when the target language monolingual data is limited. They also showed that mBART25 performs at an acceptable level even with fine-tuning for languages that did not appear in the pre-training corpora,and language relatedness has a noticeable role to play here.
~\cite{liu2020multilingual} carried out multilingua fine-tuning, and showed that only the many-to-En setting delivered good results with mBART25, as well as mBART50, compared to bilingual fine-tuning. see that the improvement from multilingual training is more significant as the quantity of training bitext decreases. 
~\citet{fan2021beyond} further explored many-to-many fine-tuning in a non-English setup, and showed that this setup outperforms bilingual fine-tuning. 
\citet{liu-etal-2021-continual} provided a preliminary comparison between mBART50 and mT5, and showed that mBART50 outperforms mT5 is all but one translation instance.
\sr{Sarui, David - anything else?}

\subsection{Empirical Evaluations on NMT Systems}
Although not for pre-trained sequence-to-sequence models, there has been many empirical research on evaluating various NMT models. \\
~\citet{zhou2021family} trained a multilingual NMT using a set of related languages, where each language had about 1000 sentences. Then this model was fine-tuned on the target language pair, which also had about 1000 sentences. They tested for the scenarios where the train/test domains are same, and different.~\citet{dabre2017empirical} evaluated the effectiveness of Transfer learning, and concluded that using a resource rich language
pair to transfer into a low-resource language pair is effective when the two source languages are linguistically similar.~\citet{mueller-etal-2020-analysis} analysed the impact of number of languages, size of the parallel corpora, and language relatedness in multilingual domain-specific NMT.~\citet{hokamp2019evaluating} evaluated the performance of many-to-many NMT models wrt training data amounts, diversity of languages, as well as domain difference between training and testing data.  

==> not used/xtra_information.tex <==
Gmail:
lowresourcenmt@gmail.com
password: lrlnmt@2021
GitHub:
Username: LRLNMT
password: lrlnmt@2021

==> sections/1.introduction.tex <==
\section{Introduction}
\label{intro}

Multilingual autoencoder-based sequence-to-sequence (MASS) models such as mBART and mT5 deliver impressive results for natural language inference, question answering, and text simplification. Their performance on machine translation (MT) is of particular interest. To avoid the time and expense of training a new model from scratch, MASS models can leverage their massive pre-training data and strong initial parameters (CITE).Their massive pre-training data can give a strong starting point for fine-tuning the model parameters toward the language and domain of interest, sparing the time and expense of training a model from scratch. MASS models show promise in the challenging context of low-resource languages  \citep{liu-etal-2021-continual}.

When can mBART and mT5 succeed in translating a low-resource language? Despite their promise, we do not know what makes these models tick. Understanding their sensitivity to dataset size, domain, and language relatedness is crucial for applying MASS models to new languages.

% Emergency situations motivate machine translation (MT) models learned from mere thousands of parallel sentences~\cite{strassel-tracey-2016-lorelei,berard-etal-2020-multilingual}.  Despite this need, neural MT (NMT) for low-resource languages (LRLs) is still a challenge~\cite{koehn-knowles-2017-six,ranathunga2021neural}.
% Multilingual pre-trained Transformer models are a promising solution for LRLs, due to their zero-shot and few-shot learning capabilities. In particular, multilingual sequence-to-sequence (seq2seq) models (e.g., mBART\footnote{There are two mBART versions: mBART25 and mBART50. This paper refers to the latter.}~\cite{tang2020multilingual} and mT5~\cite{xue2021mt5}) perform well in the context of LRLs~\cite{adelani-etal-2021-effect,liu-etal-2021-continual}, even for non-English-centric translation~\cite{cahyawijaya2021indonlg,madaan2020transfer,thillainathan2021fine}. Still, while encoder-based multilingual pre-trained models \citep{devlin2019bert,conneau2019unsupervised} have been extensively analysed with respect to LRLs~\cite{hu2020xtreme, wu2020all}, no extensive evaluation characterizes their seq2seq counterparts.

%%In general, Seq2Seq models are trained in a self-supervised manner using large-scale monolingual data; here, the monolingual data is noised and fed as a source task and original monolingual data as the target task. At the end of the self-supervised training, the trained model can take a partially noised input and predict the denoised words to recover the original sentence.  This approach strongly learns a good universal language representation from the monolingual data by capturing linguistic characteristics, lexical meanings, and syntactic and semantic structures. 

%% BART (Bidirectional and Auto-Regressive
%Transformers) was the first pre-trained model trained in this manner~\cite{lewis2019bart}. It is implemented as a standard sequence-to-sequence Transformer architecture with a bidirectional auto-encoder and a left-to-right auto aggressive decoder. Hence, it comprises two pre-trained models, a bidirectional encoder and a left-to-right decoder. mBART25~\cite{liu2020multilingual_mbart25} is the multilingual version of BART. mBART25 was later extended to cover 50 languages, resulting in the mBART 50 model (refered to as mBART hereafter)~\cite{tang2020multilingual_mbart50}.
%\sr{David - a little bit on mT5}

%%~\cite{liu2020multilingual} showed that the mBART25 model fails to deliver meaningful results when fine-tuning with less than 10k sentences. The performance has also dropped when fine-tuned with 25M sentences. They showed that pre-training on more languages helps most when the target language monolingual data is limited. They also showed that mBART25 performs at an acceptable level even with fine-tuning for languages that did not appear in the pre-training corpora,and language relatedness has a noticeable role to play here.
%~\cite{liu2020multilingual} carried out multilingual fine-tuning, and showed that only the many-to-En setting delivered good results with mBART25, as well as mBART50, compared to bilingual fine-tuning. see that the improvement from multilingual training is more significant as the quantity of training bitext decreases. 
%~\citet{fan2021beyond} further explored many-to-many fine-tuning in a non-English setup, and showed that this setup outperforms bilingual fine-tuning. 
%\citet{liu-etal-2021-continual} provided a preliminary comparison between mBART50 and mT5, and showed that mBART50 outperforms mT5 is all but one translation instance.

% In this paper, we investigate the robustness of pre-trained seq2seq models (namely, mBART due to preliminary experiments) for translating LRLs, when fine-tuned with either small amounts of manually curated domain-specific data or comparatively large amounts of noisy parallel data. We test both types of fine-tuning with domain-specific and open-domain test sets.

In this paper, we introduce a large-scale study of mBART's viability for low-resource MT. Our experiments span 10 typologically and geographically varied languages, where 8 are considered low-resource languages and 4 of which are unseen. Through our experimental results, we gauge the importance of five dimensions of the training data:

\begin{enumerate}[noitemsep]
\item Amount of fine-tuning data
\item Noise in fine-tuning data \rs{random thought...can we call just data `quality'? Noisiness is wordy} \arya{Quality is broad... How about just `noise'?}
\item Amount of pre-training data
\item Domain relatedness
\item Language relatedness
\end{enumerate}
The described five dimensions are inspired by previous works suggesting training data curation (cite something on pre-train and fine-tune data quality and quantity papers), domain adaptation (cite), and linguistic properties (cite) are influential to the poor performance on extremely low-resource languages in a non-straightforward way. The closest work to ours \citep{liu-etal-2021-continual} considers only the first two. 

Our experiments show for the seen languages, mBART reached acceptable performance with either 10k high-quality in-domain sentence pairs or 100k noisy ones.
However, mBART's performance for unseen languages is often below 3.0---far below usability. Our discovery suggests the need to explore better training strategies on MASS models to adapt to new languages \citep{thompson-etal-2018-freezing,ebrahimi-kann-2021-adapt}.

% Next, \cref{dataselection} discusses the languages and the dataset selected concerning the five factors. Followed by \cref{experimentsetup} which decouples the five factors into experiment scenarios to train the mBART model.

 %After an initial analysis of the performance of mBART50 (referred TO as mBART hereafter) and mT5, we picked the former for further experiments. 
%We consider the problem of data scarcity faced by low-resource languages and analyse the performance of pre-trained NMT models when fine-tuned with the  use of publicly available parallel data. We selected mBART50~\cite{tang2020multilingual_mbart50} model, as it is the most used model for Machine Translation, plus it has been reported to perform better on average, when compared to mT5~\cite{liu2021continual}. 
%Our analysis is guided by the observation that the publicly available parallel datasets for Machine Translation (MT)~\cite{tiedemann-thottingal-2020-opus} can be broadly categorised as (1) manually curated high quality datasets, which are small in size and are mostly domain-specific, and (2) Automatically extracted from public domain documents in the web, which are large in size but very much noisy. 
%In this study, we investigate the capability of these pre-trained models to produce robust 
% \eal{multi-}\st{shouldn't be multi-NMT, each direction is trained as separate bilingual manner}\eal{ok, resolve}
%NMT  models for low resource languages, when fine-tuned with small amounts of manually curated domain-specific data as well as comparatively large amounts noisy parallel data. Both types of fine-tuning have been tested with domain-specific, as well as open domain test data. 

%Given that mBART50 covers only 50 languages, we investigate the possibility of using mBART50 for languages not included in pre-training.
% \eal{maybe too much detail?  perhaps we can generally explain the contribution of our work in the intro and go into the logical details of the choices in the methodology}
% We find that the performance of mBART on LRLs depends on a combination of the above factors. 
% However, i


%The contributions of this paper is in 3-folds:  1) extreme LRL originating from South Asia (Sinhala, Tamil, Kannada, Assamese) and Africa (Afrikaans, isiXhosa, Yoruba). 2) empirical evidence on factors effecting mBART fine-tuning (transfer learning) of LRL (domain-specific fine-tuning, amount of data needed, generic open-domain fine-tuning, in/not-in mbart) 3) recommendations on leveraging these factors for mBart of LRL.




==> sections/2.data.tex <==
%\section{Materials and Methods}
%This section briefly discusses our experimental setup. Section \ref{dataselection} and \ref{datasetsize} explain \eal{our} low-resource languages of interest and the training set size, followed by Section \ref{domain} which discusses the domain type selection, and lastly, Section \ref{curation} explains curation factor of the evaluation. %Our experiment seeks to answer the following questions for low-resource language: ``(1) How robust is mBart when it is fine-tuned on noisy large open-domain parallel data? (2) How robust is mBART when it is fine-tuned on small domain-specific hand-curated parellel data?'' We define four driving factors that influences the domain adaptation task for low-resource languages in the below sections. 

% \eal{we need to emphasize the most important findings (discussion and results), the ordering of methodology here need to reflect that.  I am not sure "represented in mBART" is a significant result right now.}

\section{Data and Models}
\label{dataselection}

\begin{comment}
In this section, we discuss the language selection and the dataset selection for each language, and then we briefly describe the model selection for evaluating the five factors proposed in~\cref{intro}.

We selected a set of high- and low-resource languages to maximize typological and geographical diversity. Of the ten languages, five do not use the Latin script, to evaluate the generalization of large pre-trained models to non-Latin scripts \citep[see][]{pires-etal-2019-multilingual}. Eight can be considered LRLs based on \citet{joshi-etal-2020-state}, and \lang{fr} and \lang{hi} are high-resource languages to give a skyline of performance. The languages are given in \cref{tab:lang-details}.
\end{comment}

% The datasets selected for the chosen languages are shown in . 

Because open-domain datasets contain noise especially for LRLs~\cite{qualityAtAGlance}, we select both open-domain and domain-specific datasets (shown in \autoref{tab:data-details}) to evaluate the effect of fine-tuning data noise and domain relatedness. The FLORES datasets, ~\cite[\textsc{Flores}-101]{goyal2021flores} and ~\cite[\textsc{Flores}v1]{guzman2019flores} (only for Sinhala), and the automatically aligned parallel texts from Common Crawl (CC),~\cite[CCMatrix]{schwenk2019ccmatrix} and the more recent collection~\cite[CCAligned]{el2020massive}, are selected for the open-domain evaluation. Our five domain-specific datasets include religious, administrative, news, and legal domains. Although JW300 was also automatically aligned, its quality for \textit{\lang{af}, \lang{yo}, \lang{xh}} is reported to be very high~\cite{abbott2019benchmarking,alabi-etal-2020-massive}. Further details of the corpora are in \cref{app:appendix}.

% \input{table_lang_details}
% \input{table_data_details}
% \input{table_mBARTmT5}
% Aside from CC, all corpora are of high quality for the languages under study.


% , and are typically noisy for LRLs
% plus five curated, domain-specific datasets from religious, administrative, news, and legal domains. We additionally use , from the open-domain for evaluation. 
% The open domain training datasets were 
%\textbf{Resourcefulness of the language:} 
%$As for languages included in mBART, \textit{resourcefulness} was measured using the amount of language data used in the pre-training stage. As for languages that are not included in  mBART, we focused on languages belonging to 0-2 classes. These languages belong to typologically different language families, and have different writing scripts. The are distributed across three geographical areas in the world.
%\subsection{Language Selection}

% Languages in this study, with number of pre-training tokens in mBART
%  (mBART Tokens=\# of pre-training tokens)


%In the field of Neural Machine Translation, a low-resource language pair refers to a pair of languages that does not have parallel data in sufficient quantities.`\citet{ranathunga2021neural}noted that there is no definite size of parallel corpus to determine whether a language pair is low resource. When selecting languages, we needed to identify languages that are included in mBART50, and those that are not. As for the former type of languages, we consider languages that are under-represented in the mBART50 model. These languages belong to categories 0-3 in~\citet{joshi2020state}'s language categorisation. As for languages that are not included in the mBART50 model, we focused on languages belonging to 0-2 categories in \citet{joshi2020state}'s categorisation. 

%\textbf{Language Relatedness: }With the hope of analysing the performance with respect to language relatedness, we wanted to select languages belonging to different language families.

%\textbf{Data Availability:} 
%Our initial objective was to identify a set of languages that has parallel data in a common set of different domains. However, this requirement could be satisfied only with Bible data, which has data from 1600+ languages~\cite{mccarthy-etal-2020-johns} (see Table~\ref{tab:lang-details}). Thus, considering the availability of domain-specific data, we identified languages that share some common domain-specific dataset with at least one other language.  For open domain, we focused on the \textsc{Flores} evaluation dataset, which has manually curated data from 101 languages~\cite{goyal2021flores} except for Sinhala we used earlier \textsc{Flores}v1 \cite{guzman2019flores} dataset.
% \sr{sarubi - add a footnote on the other flores dataset for \lang{\lang{si}}} 
%All the languages we selected are included in the \textsc{Flores} dataset, which guarantees a common and high quality test bed for open-domain evaluation, which guarantees a reliable analysis~\cite{liu2020multilingual}. For open-domain fine-tuning data, we considered languages included in either the CCAligned~\cite{el2020massive} or CCMatrix~\cite{schwenk2019ccmatrix} datasets (hereafter referred to as CC). \\
%Table~\ref{tab:data-details} shows the datasets we used and their domains and language coverage. \textsc{Flores}, Government, PMIndia and DGT-TM are high-quality hand-curated datasets. JW300 is automatically extracted. However,~\citet{abbott2019benchmarking} manually verified that its quality for \textit{\lang{af}} and \textit{\lang{yo}} are really high. Further details of these corpora can be found in the appendix.   

%\textbf{~\cite{liu2020multilingual}  highlight the importance of using high quality evaluation datasets. Normally LRL training data is noisy.}

%As shown in Table \ref{tab:dataset}, we selected eight low-resource languages. In addition, we selected French and Hindi as two high resource languages. This is to analyse the impact of pre-training dataset size in the mBART50 model. 
%These five languages often have poor quality and limited data for the translation task \rs{need citation}, which makes them a good candidate set to evaluate mBART against the proposed evaluation factors. For each language, we experimented with both directions: from English to the low-resource language, and from the low-resource language to English. 


%\subsection{Corpus Selection}
%\label{corpus}
%The experiments use the following corpora. Table xx shows the domains of the corpora, and the experiment languages that belong to each of these corpus.

==> sections/3.setup.tex <==
\section{Experimental Settings}
\label{experimentsetup}
% \subsection{mBART or mT5: Preliminary results}
We conducted a preliminary experiment to compare mBART and mT5. Consistent with~\citet{liu-etal-2021-continual}, our results in \autoref{tab:mbartvsmt5} show that mBART performs better than mT5 on more translation directions, in particular for \lang{\lang{en}}→xx directions. Given the improved performance and the reduced computation needs, we focus hereafter on mBART.  

% This observation is consistent with~\citet{liu-etal-2021-continual}. %Interestingly, for \lang{ga}, which is included in mT5 but not in mBART, mBART outperforms mT5 for \textit{\lang{\lang{en}}→\lang{ga}}.
%Our experiments aim to evaluate the model robustness by measuring the quality of open-domain and closed-domain \rs{is it closed-domain instead of close-domain?} translation on the standard hand-crafted open-domain Flores test sets and \rs{government bible}, respectively. \cite{}. 

The language set in \cref{tab:lang-details} includes both languages used in pre-training mBART and unseen languages.
For the four unseen languages, we applied the related language fine-tuning strategy \cite{madaan2020transfer,cahyawijaya2021indonlg}. Considering syntactic closeness and language family \cite{wals, littell-etal-2017-uriel}, we picked \lang{bn} for \lang{as}, \lang{te} for \lang{kn}, \lang{fr} for \lang{ga}, and \lang{sw} for \lang{yo}. 

We compare mBART to the standard Transformer \citep{vaswani2017attention} to baseline the value of pre-training.
% We fine-tuned mBART with (1) domain-specific data and (2) automatically aligned parallel data from bitext mining, where the former has high quality and the latter is substantially noiser. 
% Because fine-tuning mBART would update the model parameters \rs{better wording}, 
We measure the performance difference in fine-tuning on open-domain and domain-specific datasets to uncover mBART's sensitivity to data quality and domain relatedness. We discuss the fine-tuning datasets in \cref{ftprocedure}, and the rest experimental details of all the fine-tuned models are included in \cref{app:appendix}.
% We compared the performance when it is fine-tuned with high quality domain-specific data or automatically aligned noisy parallel data from bitext mining. 


\subsection{Fine-tuning Dataset}
\label{ftprocedure}
% \paragraph{Noisy Open-Domain Data} 
    
Open-domain data are more easily available than close-domain data. Although at the cost of data quality. For most of the languages, CC datasets contain more than 100k sentences, making them much larger than the domain-specific datasets. Considering the common largest dataset sizes for the selected languages, we selected two dataset sizes: 100k and 25k parallel sentences.\footnote{Assamese only has around 25k sentences.} We used \textsc{Flores} as the dev set and tested on \textsc{Flores}'s test set, plus two other domain-specific datasets.  
%Our objective was to analyse the impact of fine-tuning datset size on mBART performance. The the fine-tuned mBART50 model is evaluated on an open-domain set and two close-domain test sets. We use Flores101 as the open-domain dev/test sets, and the domain-specific dataset is as per Table xx. If the domain of data is considered, testing with the domain-specific datasets can be considered as a zero-shot case.

For each language pair, we fine-tuned mBART with two domain-specific datasets to compare the fine-tuned mBART's performance with noisy open-domain  datasets. Because the hand-curated datasets are much smaller, we vary the set size between 1k, 10k, 50k and 100k sentences. However, not all datasets come in the same size. For example, the Bible datasets for some languages (\lang{\lang{ga}},  \lang{kn}) contain only around 4k sentences. 
% For fine-tuning, 
We use the train and development sets of one domain during fine-tuning, and evaluate against the same-domain data, another domain, and \textsc{Flores} at test time. %Similar to the previous experiment, evaluation with a different domain data as well as \textsc{Flores}101 data can be considered as a zero-shot case. 

==> sections/4.analysis.tex <==
% \section{Results and Analysis}
% % In this section, we present and discuss the experimental results with respect to each evaluation dimension proposed in \cref{intro}.

% % \input{table_new}
% \footnotetext[4]{We use 25k CC for training \lang{as}.}
% % \footnotetext[5]{We use 1k for \lang{as}, 10k for \lang{kn}, and 50k for \lang{hi} for PMI}
% \footnotetext[6]{\lang{fr} results in Appendix}

% % \paragraph{Case 1. Fine-tuning with open-domain data} 

% \label{case1}

% \subsection{Amount of Fine-tuning Data} 
% % open-domain
% In the open-domain case, for languages included in mBART, fine-tuning with 25k parallel data outperforms the Transformer model trained with 100k parallel data for all the translation tasks\footnote{Except for \textit{\lang{\lang{en}}→\lang{xh}} where the two results are on par.}. Our results indicate that pre-trained mBART is at least four times as data-efficient. mBART shows better performance than the Transformer even for unseen languages, although the results are not significant. \rs{why are we saying it's better if it's not significant? could this be a footnote too?}
% % Specifically, for Yoruba, the performance is noticeably improved when the fine-tuning dataset size reaches 100k.

% % close domain
% % When training with domain-specific datasets (Gov't, JW300, and DGT), 
% We observe a similar trend for data efficiency for mBART (compared with the Transformer model) when training with domain-specific datasets (Gov't, JW300, and DGT). 
% % With 10k sentences of government-domain parallel data, 
% For the government-domain dataset, mBART trained with 10k sentences outperforms the Transformer trained with 50k sentences, which suggests a five-fold data efficiency.\footnote{Except with \textit{\lang{\lang{en}}-\lang{\lang{ta}}}, where the result is on par.} 
% For JW300, mBART trained with 10k parallel sentences outperforms the Transformer trained with 100k for some translation tasks by ten-fold.
% Further, mBART trained with 50k sentences outperforms the Transformer model for all the languages by five-fold.\footnote{Except with \textit{\lang{\lang{en}}-\lang{xh}} in-domain testing, which is on par.} 

% \rs{move to conclusion?}
% Thus, for these domain-specific datasets, mBART might outperform standard Transformers by an efficiency of five to ten times; 
% future work can pinpoint the saturation size.
% This is even more prominent for inference on unseen languages. Fine-tuned mBART is robust to domain differences, while the transformer flounders for out-domain datasets. % (100k:10k jw300 and 50k:10k gov).


% \autoref{fig:fine-tuning_size} shows the impact of fine-tuning dataset size. Although training with more data improves model performance, the gain gradually saturates as the dataset size reaches around 50k. \citet{liu2020multilingual_mbart25} attributed this observation to the model capacity issue, that the pre-trained weights are slowly ``washed-out'' when fine-tuning with more parallel data.% explained this phenomenon that when more parallel data is provided, the supervised training would gradually wash out the pre-trained weights.
% % \sn{Surangika- This might be a good explanation for the results of ka and \lang{ta}. 
% % The Dravidian languages are all agglutinative, making inward
% % translation challenging, but also making the evaluation of translation using word-based metrics like BLEU less reliable\cite{Barry2020PMIndia}.}\eal{note this is cut and pasted from the paper, "agglutinative" is a big word, please reword, thank you!}
% \begin{figure}[t]
% \includegraphics[width=\linewidth]{images/domainrelated_finetuningsize.png}
% \caption{Impact of fine-tuning dataset size on mBART performance for JW300 in one translation directions}
% \vspace{-2mm}
% \label{fig:fine-tuning_size}
% \end{figure}


% \subsection{Noisiness of Fine-tuning Data}  
% % open-domain
% Although CC data includes all the selected languages in equal amounts, the quality of these automatically extracted datasets is not guaranteed. Especially in the case for low-resource languages~\citet{qualityAtAGlance}.
% % showed that automatically extracted data is noisier for LRLs, which explains the low results on LRLs. 
% This phenomenon crucially contributes to the poor results (shown in \autoref{tab:result-lk-eu}) in the Transformer model in the low-resource setting. 
% Further, this highlights a vicious cycle that the automatic bitext mining techniques for LRLs are built on insufficient parallel data or high-quality monolingual data \rs{should it be low quality?}, which 
% in turn 
% % results in 
% % these models extracting 
% provides noisy parallel data to the downstream translation task. 
% % NMT models trained with these noisy data have low performance. 
% \rs{is is a factor in the close-domain case too?}

% \subsection{Amount of Pre-training Data}  
% %mBART does not treat all the languages equally. 
% As shown in \autoref{fig:pretraining_size}, mBART performs better compared to
% % shows that the performance comparison between mBART and 
% the Transformer model and the gain is more prominent as the amount of pre-training data increases ($R^2=0.31$).
% %This result shows that languages that have higher amounts of data during mBART pre-training have a strong gain over the other LRLs. 
% % \begin{figure}[t]
% % \includegraphics[width=\linewidth]{images/mBART_pre-training_gains.png}
% % \caption{Effect of the pre-training open-domain dataset size}
% % \vspace{-2mm}
% % \label{fig:pretraining_size}
% % \end{figure}
% \rs{is this fig just for open-domain case, or for both? The explanation for closed-domain is just it's the same}
% Similar effect is observed for the domain-specific case. 
% % closed-domain
% The impact of pre-training set size shows a trend similar to Case 1: languages with a higher representation in mBART have clear gains over the LRLs. \rs{what does this mean?}
% \subsection{Domain Relatedness} 
% % open domain
% mBART trained on Bible data shows a consistently lower performance across all experiments. We attribute this to the domain difference between CC and Bible data.
% \sr{annie - give some divergent stats to match here}. \eal{What we could say is the fine-tuing cc performs better for ccalign, the third domain, the finally the Bible; which we cannot explain because Bible is actually closer than the 3rd domain}\\
% Surprisingly, we notice the impact of domain-relatedness between the training and testing parallel data. The
% \eal{case 1 conclusions:  1. mBART is at least four times as efficient with respect to data requirements; 2. vicious cycle of poor cc data for lrl}

% \paragraph{Case 2. Fine-tuning  with  domain-specific data}




% closed-domain
% \paragraph{Domain relatedness.} 
For the government dataset, \lang{en}→\lang{si}  and \lang{en}→\lang{ta} get 11.2 and 6.6 BLEU (respectively) for same-domain translation when fine-tuned with just 1k parallel sentences.
\rs{not sure if this is actually good results. Could we say: mBART trained on 10k sentences achieved higher performance compared with the transformer trained on 50/100k data, suggesting the pre-trained gain was able to compensate the lack of in-domain data?}

Results for translating into English are even higher for both languages. This may indicate the utility of mBART for domain-specific translation with low amounts of high-quality data. 
% However, 
\rs{this is a bit scattered imo}
We believe this result depends on either the high-quality English language model manifest in the decoder, or the domain relatedness between the language data in mBART and fine-tuning data: for Bible, \lang{en}→\lang{si} and \lang{si}→\lang{en} reach only 3.6 and 9 BLEU, respectively. Results for \lang{fr} on the DGT and Bible data, and results for \lang{hi} on PMI data  suggest that mBART provides better results when fine-tuned with even 1k parallel sentences, if the language has sufficient coverage in mBART.%   \eal{can we say something generic overall for all the in/out-domain test dataset?}. 
% which we attribute to the domain difference between the data in the mBART pre-trained model and the Bible. This suggests that Bible data, if only available in small quantities, may not be useful with mBART. Whether this observation changes with more Bible data should be subjected to more experiments. However, the same issue does not hold for \textit{\lang{fr}}, which has comparably higher coverage in mBART. \eal{I think maybe we need to say Bible has similar vocabulary but maybe the sentence structure is different?}
Performance of mBART on out-domain is much less when fine-tuned with just 1k parallel data, even for languages in the model. The actual performance depends on the relatedness between the two domains. For example, training on the government dataset, in-domain translation obtains 14.78 BLEU, whereas \textsc{Flores} and Bible only obtain 6.52 and 2.48 BLEU (respectively); domain of the latter is more different from the government domain. On the other hand, if data from a different domain is available in sufficient quantities, an acceptable translation performance can be expected, as evident by the mBART models fine-tuned with government 50k data or JW300 100k data. 
Noticeably, issues related to domain difference and fine-tuning dataset size are less pronounced for \textit{\lang{fr}} (see results for 1k Bible data and 1k DGT). This highlights the impact of language coverage in the mBART model.  

\begin{comment}
\subsection{Language Relatedness} 
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/syn_sim.pdf}
%     \caption{Cosine similarities of syntactic features}
%     \label{fig:syn_sim}
% \end{figure}
% what we found
We observe a much higher performance for \lang{\lang{af}} compared with other LRLs that were used to pre-train mBART across most experiments.
Similar to~\citet{zhou-waibel-2021-family}, we attribute this performance gain to \lang{\lang{af}}'s relationship with \lang{\lang{en}}: both are Germanic and share the Latin script. 
Our results are consistent with ~\cite{zhou-waibel-2021-family}, whom has also noticed exceptionally high performance for \textit{\lang{en}-\lang{af}} translation.
% what we believe
Previous works suggest that multilingual machine translation systems can learn shared representations for linguistically similar languages~\cite{neubig-hu-2018-rapid, kudugunta-etal-2019-investigating}\rs{add more if we need}. Specifically, \citet{neubig-hu-2018-rapid} shows that empirically, adapting NMT to new languages benefit from training with high resource languages that are topologically similar or having a large amount of lexical overlap. In addition, \citet{arivazhagan2019massively} found that by using a smaller token set has a larger improvement on the LRL due to improved generalization. \rs{ref back to table 1}. Word order might also play a crucial factor (\lang{\lang{ga}}: VSO; \lang{\lang{af}}: SVO) in distinguishing the performance between the LRL and the HRLs, even when they are lexically similar \cite{Liu_Winata_Cahyawijaya_Madotto_Lin_Fung_2021}.

% what we found for unseen
On the other hand, mBART's performance is less trivial for \textit{unseen} languages that share the Latin script with English.
For example, the performance in \lang{\lang{yo}} is better than \lang{\lang{ga}} despite both languages use Latin script.    
% what we believe
To uncover the performance between \lang{\lang{af}} and \lang{\lang{ga}}, we use the syntactic features estimated by the \textit{k}-nearest neighbors ~\cite{littell-etal-2017-uriel} using the existing WALS syntactic features~\cite{wals}. \Cref{fig:syn_sim} shows the syntactic similarities between the two languages of interest with three other high resource languages. It is possible that \lang{\lang{af}} is more syntactically similar to high resource languages (such as \lang{\lang{en}}, \lang{\lang{de}}, and \lang{\lang{nl}}) than \lang{\lang{ga}}.
% We hypothesize that the result is exceptionally high for the 1k fine-tuning case for both datasets because the fine-tuning does not override the strong model weights from pre-training.  
% In general, \textit{\lang{af}} has exceptionally high results across most of the experiments. We believe this is due to its high similarity with English. 
% \eal{Rosaline, is \lang{en} closer to \lang{af} than \lang{fr}?  What are the closest langages to \lang{af}?  We can add this back} \rs{
% Linguistically, \textit{\lang{en}} is slightly closer to \textit{\lang{af}} (0.84) 
% syntactically compared with French (0.77). Yoruba is not as close to these high resource langs as compared to \lang{af}, maybe that makes a difference? 

% \eal{remove?}
% The impact of language relatedness is visible in the experiments related to government dataset as well. Despite having low amounts of data in the mBART model, \textit{\lang{si}} performs better than \textit{\lang{ta}}. Interestingly, the transformer results for the two languages are more or less the same. Given that mBART includes for Indo-European languages s.a. \textit{\lang{si}} than Dravidian languages s.a. \textit{\lang{ta}}, we can conclude that \textit{\lang{si}} gets the support from more related languages than \textit{\lang{ta}}.~\citet{hu2020xtreme} noticed the same in mBERT and XLM-R models.
% \eal{I think because it is only about 2 languages, we could move to appendix?  Unless David, could we make similar observations for African languages; Shravan can we make similar observations for Indian languages? For Rosaline/Arya to comment further}

\section{Conclusion}
When limited parallel corpora are available, fine-tuning mBART can improve translation performance over training transformers from scratch. 
Our proposed five factors uncover the relationship between mBART's performance and what is available for the low-resource data. 
%:  language coverage in the mBART pre-training, fine-tuning dataset size, domain relatedness between training and testing data, domain relatedness between pre-training and fine-tuning data language relatedness, and the noisiness of data. 
%Our observations in fine-tuning mBART indicate that translating in low-resource setting should be scrutinized with respect to data quantity, quality, and closeness. 
In the future, we hope to investigate curricula and data augmentation so mBART does not struggle on unseen languages, which will help in low-resource scenarios. 
% Despite the variance in results, our observations can serve as practical recommendations when using mBART for LRL translation. 
%For example, in our open-domain experiments, we found that fine-tuning mBART achieves a four-fold data-efficiency gain for both languages in and not in the original mBART model pre-training.  Similarly in our domain-specific experiments, we found that fine-tuning mBART achieves a five-fold data-efficiency.  
%\footnote{For example, even 1k parallel in-domain data (e.g.~ for \textit{\lang{en}-\lang{si}} in-domain translation with domain-speicifc government data) would be enough to derive an acceptable translation model from mBART.  As for languages not covered in mBART, \textit{yo} can yield reasonable results when 100k high quality parallel data is available. For the other three LRLs (\textit{as, ka, ga}), mBART performance is not at a usable level. This could be due to the nuances in language script and pre-processing mechanisms in the hugginface library we used~\footnote{For example, \textit{ka} is known to have a zero-width joiner issue \url{https://github.com/google/sentencepiece/issues/629}}. A closer examination on this is issue required to identify the exact problem.}  Our results also imply that the more fine-tuning data, the better the results, and in-domain testing that matches the fine-tuning dataset outperforms out-of-domain testing. \eal{this sentence is a little obvious...so not sure if it is needed; consider removing to save space, there was also a paragraph on this in the results analysis we can remove}


%While our preliminary study makes some initial observations, further study into factors such as language and domain relatedness and theoretical proof is needed to draw out more concrete conclusions\sr{will this be a negative }.  %We tested with varying sizes of parallel sentences; however, if more data is available it is worth experimenting to see whether there exists a saturation in dataset size. This is important as fine-tuning mBART model is memory extensive.
\end{comment}

\iffalse
\subsection{Results Analysis}


\eal{OBSERVATIONS (Point form for now...will refine later.):}
\subsubsection{Analysis 1. expr2 domain-relatedness training mBART for LRL}
\begin{itemize}
    \item in-domain >> out-domain testing (except \lang{af} Bible, finetuning 1k not sufficient to outweight pretraining): jw300, afrikan very good, larger size always better, yo is important because results are always better than transformer; in-domain better than out-domain (even 1k gives noticable better results); same for government and Bible results are low due to domain difference, 
    \item data efficiency (both directions):  expect data requirement in mBart always less than transformer (depends on the domain) about 1/4 25 percent.  mbart 50k << transformer 100k (sometimes even 10k for example yo train JW300, test FLORES and JW300 and xh test FLORES); similarly gov 10k mbart >> 50k transformer; when compare ccalign 100k transformer << mbart 25k; 
    \item Bible domain:  mbart vs transformer: very little data in Bible 1k  low performance for both transformer and mBart (usually below 1 BLEU); however when testset is Bible, mBart always better than transformer (> 1 BLEU); in-domain Bible >> out-domain; results always lower for languages not in mBart
    \item data efficiency is more prominent for out-of-domain:  transformer performs poorly for out-domain datasets (100:10 jw300 and 50:10 gov) for out-domain mBART has more data efficiency power than transformer when trying "adapt" to a different domain; domain relatedness matters a lot
    \item special case:  the Afrikan exception for Bible 1k promising results (related to English and Dutch), data in mBART is relaetd to flores and jw300 compared to Bible (pre-train model >> fine-tune Bible), not enough fine-tuning taking place so assume \lang{af} 
    \item data efficiency in/not-in mbart:  for in-domain 50k does much better than transformer 100k (yo jw300)
\begin{itemize}
\end{itemize}
    \item transformer can explain the relatedness between \lang{en} -> xx, get quality of the training set; that's why extreme lrl have very low results
    \item transform results flores >> domain-specific, mbart is vice-versa; transformer is trained from scratch but mbart is pre-trained and some preliminary information might already be there in the pre-trained mbart model
    \item in/not-in mbart, even some small amount of fine-tuning paralel text for mbart, it always gives better results than simple transformer
    \item mbart better than mt5,  \eal{Shravan to add table and experimental setup}
    % \item \eal{consult with team, a linear graph on translation results v.s. domain relatedness}
    % \item \eal{consult with team other visualizations, such as  heatmap by specific "surprising" languages?}
\end{itemize}

\subsubsection{Analysis 2. size}
\begin{itemize}
    \item 25k results are all better than 100k (parallel better results), even languages not in mbart transformer
    \item correlation between fine-tuning dataset (i.e. 25k v.s. 100k for mbart and for transformer)
    \item surprising observation that we cannot explain: 50k sometimes better than 100k?  further hypothesis required and need further examination;  (maybe next paper?)
    \item 1k-10k noticible gain, 10-50k often gain, 50-100k hard to see; catestrophic forgetting (fine-tuning stage) \eal{David can bring this out more}

\end{itemize}

\subsubsection{Analysis 3. noisines of ccalign}
\begin{itemize}
    \itme \eal{surangika please add something}
\end{itemize}

\subsubsection{Analysis 4. domain relatedness}
\begin{itemize}
    \item surprisingly, NIV Bible is similar to open domain (FLORES and then CCALIGN), but it trains very poorly compared to the other domain-specific datasets (i.e. jw300, DGT, PMO, government).  See figure below.  Bible tend to perform worst than others; generally one side better than other; Bible tend to perform worst than others; generally one side better than other
    \item ccalign results:  usually Bible < Domain 3 < Flores; note that ccalign may also contain jw300 (thus explaining why jw300 is better for Xhosa and maybe Yoruba which is just a little, so we can see domain relatedness between jw300 and ccalign is >1); because it is in the training).  UNEXPLAINED:  For Government Sihala > Tamil quality, pehraps government tamil is similar?  But Gov is similar to ccalign?
    \item ccalign experiment:  cclaing-gov is closer than ccalign/flores \eal{surangika to discuss \lang{si} > tm}
    \item Domain-relatedness for the ccalign dataset: French and Assamese is the most different followed by French.  The Indic languages (Tamil, Sinhala, Kannada, and Hinda ) are similar to one another.  French is very different as well Assamese.
    \item The dataset that is the most common overall with others is the "flores" followed by "CCALIGN", which are both open datasets (except for ccalign french).  The dastest that is the most different is the DGT (especially french), followed by the jw300.  See figure below.
\end{itemize}


\subsubsection{Analysis 5. Other observations and unexplained surprises}
\begin{itemize}
    \item xx-->\lang{en} always better, because all multiple languages anchored in English so there is more English data
    \item domain-specific experiment 2:  related train-test always better, bigger size always better, except for 50-100k for French
    \item domain-specific experiment 2 (in green) xx->\lang{en}:  Hindi more data for pretrained than Sinhala
    \item unreasonably good results for Afrikaans \eal{David to explain}
    \item The Dravidian languages (ka, \lang{ta}) are agglutinative (concepts are expressed in complex words consisting many elements, rather than by inflection or by using isolated elements). Hence \lang{en}-xx translation is difficult.
    \item More domain specific the dataset better the mt results??
\end{itemize}
\fi
